Are Code Review Processes Influenced by the Genders of the Participants?

Background: Contemporary software development organizations lack diversity and the ratios of women in Free and open-source software (FOSS) communities are even lower than the industry average. Although the results of recent studies hint the existence of biases against women, it is unclear to what extent such biases influence the outcomes of software development tasks. Objective: This study aims to conceptually replicate two recent studies investigating gender biases in FOSS communities \textit{ to identify whether the outcomes of or participation in code reviews (or pull requests) are influenced by the gender of a developer.} In particular, this study focuses on two outcome aspects (i.e., code acceptance, and review interval) and one participation aspect (i.e., code review participation) of code review processes. Method: We will augment the dataset used in the original studies with code reviews /pull requests created during recent years. Using this dataset, we will train multivariate regression models to accurately model the influences of developers' genders on code acceptance, review intervals, and code review participation.

==> Sections/conclusion.tex <==
\section{Analysis plan}\label{conclusion}

\subsection{Descriptive Statistics:} We will present the mean, and standard deviation of demographics of non-casual developers, dependent and independent variables of our study. We will also present a correlation matrix between the variables to examine their relationships and covariance.


\subsection{Validity Threats:}




